Fixed Point Certificates for Reachability and Expected Rewards in MDPs

The possibility of errors in human-engineered formal verification software, such as model checkers, poses a serious threat to the purpose of these tools. An established approach to mitigate this problem are certificates -- lightweight, easy-to-check proofs of the verification results. In this paper, we develop novel certificates for model checking of Markov decision processes (MDPs) with quantitative reachability and expected reward properties. Our approach is conceptually simple and relies almost exclusively on elementary fixed point theory. Our certificates work for arbitrary finite MDPs and can be readily computed with little overhead using standard algorithms. We formalize the soundness of our certificates in Isabelle/HOL and provide a formally verified certificate checker. Moreover, we augment existing algorithms in the probabilistic model checker Storm with the ability to produce certificates and demonstrate practical applicability by conducting the first formal certification of the reference results in the Quantitative Verification Benchmark Set.

==> 3_qualitativeReachAndSafe-2functionApproach.tex <==
\section{Certifying Qualitative Reachability}
\label{sec:qualreachandsafe}

All results stated in \Cref{sec:qualreachandsafe}, \Cref{sec:certificates} and \Cref{sec:ExpRew} (even the ones takes from the literature) are formally proved in Isabelle/HOL.
\tw{make sure that this is actually the case. Also make this very prominent in intro/abstract.}

Our certificates for reachability ($\Cref{sec:certificates}$) and also for expected rewards ($\Cref{sec:ExpRew}$) need to validate qualitative reachability properties in certain cases. In this section, we describe how qualitative reachability can be certified in general. The certificates include a rank vector $\rank$ containing information about the maximal or minimal distance between states and the target set $\target$. In the following definition, we assume $1 + \infty = \infty$.


%Let $\exnats = \nats \cup \{\infty\}$ be the set of \emph{extended natural numbers}.
%We extend the standard order on $\nats$ to $\exnats$ by requiring that $a \leq \infty$ for all $a \in \exnats$.
%With this definition, $(\exnats, \leq)$ is a complete lattice.
%Further, we define $0 \cdot \infty = \infty \cdot 0 = 0$, and for all $a \in \exnats\setminus \{0\}$ and $b \in \exnats$ we let $a \cdot \infty = \infty \cdot a = \infty$ and $b + \infty = \infty + b = \infty$.

\begin{definition}[Distance Operators]
    \label{def:distop}
    Let $\mdptuple$ be an MDP, let $\target \subseteq \states$, and let $\optone, \opttwo \in \{\min, \max\}$.
    We define the following \emph{distance operator}:
    \begin{align*}
        \distop{\optone, \opttwo}{\target} \colon
        ~
        \exnats^\states \to \exnats^\states,
        ~
        \rank \mapsto \lambda s.
        \begin{cases}
            1 ~+~ \underset{a \in \act(s)}{\optone} ~ \underset{s' \in \post(s,a)}{\opttwo}  \rank(s') & \text{ if } s \in \states\setminus\target \\
            0 & \text{ if } s \in \target
        \end{cases}
    \end{align*}
\end{definition}

Notice that in \Cref{def:distop} we use lambda notion \enquote{$\lambda s$} to define the output vector (a function of type $\states \to \exnats$) of the distance operator for a given input.

$\distop{\optone, \opttwo}{\target}$ is a monotone function on the complete lattice $(\exnats^\states, \leq)$ and thus has a least fixed point by \Cref{thm:knastertarski}.
In fact, we even have the following:

\begin{restatable}[Unique Fixed Point]{lemma}{distopuniquefp}
\label{lem:distopuniquefp}
    $\distop{\optone, \opttwo}{\target}$ has a unique fixed point.
\end{restatable}
\tw{proof: \Cref{app:distopuniquefp}}

Intuitively, the fixed point $\rank = \fp{\distop{\optone, \opttwo}{\target}}$ characterizes the following distances when viewing the MDP as a directed graph (see \Cref{fig:exampleReach}):
\begin{itemize}
    \item For $\optone = \opttwo = \min$, $\rank(s)$ is the length of a shortest path from $s$ to $\target$, or $\infty$ if no such path exists. 
    \item For $\optone = \opttwo = \max$, $\rank(s)$ is the supremum of the lenghts of all paths from $s$ to $\target$, or $\infty$ if no such path exists.
    \item For $\optone \neq \opttwo$, \tw{todo}
\end{itemize}

\begin{itemize}
	\item Talk to others about how the dist op should look (where to put T, opt, r, s, sigma, x and the fact that it's the modified one.)
	\item Remove opt2 in Def 1, Lem 2 and Prop 1. Remove Lem 3.
	\item Lem 2 and Prop 1 do equal or greater than 0.
	\item For equal or less than 1, we use the new thing; since this uses lfp (not unique fp), we can only certify it from one direction, but that suffices. 
	\item In essence, Tim's distance operator does two things: (1) By using lfp and assigning infty to targets, it implicitly finds the set Z. (2) By having the conditional plus 1, it does not count to infty in max ECs.
	\item To make it unique, we could do the following: Find the set Z using Lem. 2. 
	Then, use the normal distance operator with Z as target set, but for max use the modified counting with Tim's fix.
\end{itemize}



\mwnote{Below needs to be adapted.}


Now we show how qualitative reachability and safety information can be read from the unique fixed point of the distance operator.
For $\opt \in \{\min, \max\}$, we use the notation $\nmin = \max$ and $\nmax = \min$.



\begin{restatable}{lemma}{distopequiv}
\label{lem:distopequiv}
    Let $\optone, \opttwo \in \{\min, \max\}$ and let $\rank = \fp{\distop{\optone, \opttwo}{\target}}$.
    Then:
    \begin{enumerate}
        \item\label{it:distopequiv1} If $\opttwo = \min$, it holds for all $s \in \states$ that $\rank(s) = \infty \iff \pr_s^{\noptone}(\lozenge \target) = 0$.
        \item\label{it:distopequiv2} If $\opttwo = \max$, it holds for all $s \in \states$ that $\rank(s) < \infty \implies \pr_s^{\noptone}(\lozenge \target) = 1$.\tw{this is incomplete. is this used anywhere?}
    \end{enumerate}
\end{restatable}
\tw{proof: \Cref{app:rankandqualreach}}

Notice the difference between $\opttwo = \min$ and $\opttwo = \max$. For $\opttwo = \max$, only the implication in one direction holds. See \Cref{app:missingDirection} for a counter example for the missing Direction. In order to obtain certificates for the missing direction\tw{??} in another way, we implement the following mechanism that uses two different distance operators. By that, the certificates will also need two ranking functions instead of one.

\begin{lemma}
\label{lem:distopequivextended}
    Let $\optone \in \{\min, \max\}$, $Z = \{s \in \states \mid \fp{\distop{\optone, \min}{\target}}(s) = \infty\}$, and let $\rank = \fp{\distop{\noptone, \min}{Z}}$.
    It holds for all $s \in \states$ that $\rank(s) = \infty \impliedby \pr_s^{\noptone}(\lozenge \target) = 1$.
\end{lemma}
\begin{proof}
    By \Cref{lem:distopequiv}.\ref{it:distopequiv1}, the set $Z$ contains precisely the states $s \in \states$ with $\pr_s^{\noptone}(\lozenge \target) = 0$.
    Now let $s \in \states$ be such that $\pr_s^{\noptone}(\lozenge \target) = 1$.
    Towards a contradiction, assume that $\pr_s^{\optone}(\lozenge Z) = \epsilon > 0$. Now, for $\optone = \min$ this means that for all strategies $\strat$, $\prind{\strat}_s(\lozenge \{s'\}) \geq \epsilon$ for some $s' \in Z$, which leads to a contradiction by the definition of $Z$. For $\optone = \max$ this means that there exists a strategy $\strat$ such that $\prind{\strat}_s(\lozenge \{s'\}) = \epsilon$ for some $s' \in Z$, which leads to a contradiction by the definition of $Z$ again.
    It follows\tw{justification for this?}\dz{Added it. Does it make sense? Maybe we can also move this proof in the appendix since it got longer when making it more precise. We are still discussing about including this Lemma anyway} that $\pr_s^{\optone}(\lozenge Z) = 0$, which is, according to \Cref{lem:distopequiv}.\ref{it:distopequiv1} again, equivalent to $\fp{\distop{\noptone, \min}{Z}}(s) = \infty$.
\end{proof}

%\twin{I think \Cref{lem:distopequivextended} is wrong, I try to give a corrected version in the following}
%\begin{lemma}
%    \label{thm:TplusZisOne}
%    Let $\mdptuple$ be a finite MDP with target set $\target \subseteq S$, and let $\opt \in \{\min, \max\}$.
%    Define $Z = \{s \in \states \mid \propt_s(\reach \target) = 0\}$.
%    Then $\propt_s(\reach \target) + \pr_s^{\nopt}(\reach Z) = 1$.
%\end{lemma}
%\begin{proof}
%    
%\end{proof}
%
%\begin{lemma}
%    Let $\mdptuple$ be a finite MDP with target set $\target \subseteq S$, and let $\opt \in \{\min, \max\}$.
%    Define $Z = \{s \in \states \mid \propt_s(\reach \target) = 0\}$.
%    Further, let $\rank = \fp{\distop{\opt, \min}{Z}}$.
%    Then for all $s \in \states$:
%    \[
%        \rank(s) = \infty
%        \iff
%        \propt_s(\reach \target) = 1
%        ~.
%    \]
%\end{lemma}
%\begin{proof}
%    \begin{align*}
%        & \rank(s) = \infty \\
%        {}\iff{} & \pr_s^{\nopt}(\reach Z) = 0 \tag{\Cref{lem:distopequiv}} \\
%        {}\iff{} & \propt_s(\reach \target) = 1 \tag{\Cref{thm:TplusZisOne}}
%    \end{align*}
%\end{proof}
%\twin{fix of \Cref{lem:distopequivextended} end}


We are ready to describe two different certificates for qualitative reachability from a certain state $s$ to the target $\target$. The certificates consist of either one or two ranking functions.
\begin{proposition}[Certifying Positive and Almost Sure Reachability]
\label{prop:certQualReach}
    Let $\mdptuple$ be an MDP with target set $\target \subseteq \states$.
    Further, let $\rank \in \exnats^\states$ and $s \in \states$. If
    \begin{enumerate}
        \item $\distop{\optone,\opttwo}{\target}(\rank) \leq \rank$, \quad \textnormal{and}
        \item $\rank(s) < \infty$,
    \end{enumerate}
    then for $\opttwo = \min$, we have that $\pr_s^{\noptone}(\lozenge \target) > 0$ and for $\opttwo = \max$, we have that $\pr_s^{\noptone}(\lozenge \target) = 1$.

\end{proposition}
\begin{proof}
    By \Cref{thm:knastertarski} (Knaster-Tarski) we have $\fp{\distop{\optone,\opttwo}{\target}}(s) \leq \rank(s) < \infty$.
    The claim then follows from \Cref{lem:distopequiv}.\ref{it:distopequiv1} and \Cref{lem:distopequiv}.\ref{it:distopequiv2} (notice that only the \enquote{$\impliedby$} direction of \Cref{lem:distopequiv}.\ref{it:distopequiv1} is needed).
\end{proof}

\begin{proposition}[Certifying Non-Almost Sure Reachability]
\label{prop:certQualReach2}
    Let $\mdp$ be a finite MDP with target set $\target \subseteq \states$.
    Further, let $\rank_1, \rank_2 \in \exnats^\states$, $\Zrankone = \{s \in \states \mid \rank_1(s) = \infty\}$ and $s \in \states$.
    If
    \begin{enumerate}
        \item $\rank_1 \leq \distop{\opt, \min}{\target}(\rank_1) ~\textnormal{and}~ \distop{\nopt, \min}{\Zrankone}(\rank_2) \leq \rank_2$, \quad \textnormal{and}
        \item $\rank_2(s) < \infty$,
    \end{enumerate}
    then $\pr_s^{\nopt}(\lozenge \target) < 1$.
\end{proposition}
\begin{proof}
    The first part of bullet 1 and Knaster-Tarski yield that
    $\rank_1 \leq \fp{\distop{\opt, \min}{\target}}$ and thus $\Zrankone \subseteq Z$ for the set $Z = \{s \in \states \mid \fp{\distop{\opt, \min}{\target}}(s) = \infty\}$.
    \Cref{lem:distopSubset} yields that $\fp{\distop{\nopt, \min}{Z}} \leq \fp{\distop{\nopt, \min}{\Zrankone}}$.
    The second part of bullet 1, Knaster-Tarski and bullet 2 yield that $\fp{\distop{\nopt, \min}{\Zrankone}}(s) \leq \rank_2(s) < \infty$. Then, the proposition follows from \Cref{lem:distopequivextended}.
\end{proof}

Apart from minimizing or maximizing, a third option for choosing the actions used by the distance operator is by explicitly giving a strategy $\strat \in \act^\states$. This yields a distance operator $\distop{\strat, \opt}{\target}$ with similar properties and certification techniques. See \Cref{app:distopstrat} for the full details regarding the distance operator dependent on a strategy.

==> 6b_complexity.tex <==
\section{Complexity and Comparison}
\label{sec:complexity}


\begin{table}[t]
\caption{Certificate size}
\begin{center}
\begin{tabular}{l|lll}
    \toprule
     & Reachability & Expected rewards $\starinf$ & Expected rewards $\starrho$ \\ \midrule
Umin & n & 2n  & n \\
Umax & n & 2n  & n \\
Lmin & 2n & 3n  & 4n \\
Lmax & 2n & 3n  & 4n \\  
\bottomrule
\end{tabular}
\end{center}
\label{tab:certsize}
\end{table}

\begin{table}[t]
\caption{Occuring problems}
\begin{center}
\begin{tabular}{l|lll}
    \toprule
     & Reachability & Expected rewards $\starinf$ & Expected rewards $\starrho$ \\ \midrule
Umin & P1 & P1,P2,P3  & P1 \\
Umax & P1 & P1,P2  & P1 \\
Lmin & P1,P2 & P1,P4  & P1,P4,P5 \\
Lmax & P1,P2,P3 & P1,P4  & P1,P3,P4,P5 \\  
\bottomrule
\end{tabular}
\end{center}
\label{tab:certsize}
\end{table}


\subsection{Complexity of Checking our Certificates}
\begin{restatable}[Size, Runtime and Space of our Certificates, Proof in \Cref{app:complexity}]{theorem}{complexity}
\label{thm:complexity}
    \begin{enumerate}
        \item Certificate size: Linearly many numbers. Discuss numbers.
        % The size of our certificates as given in \Cref{tab:certsize} is correct.
        \item Our certification algorithms \Cref{alg:checkMinLower} - \Cref{alg:checkMaxLowerExpRewRhoNoWitness} given in \Cref{sec:algs:checkingCerts} perform $O(\abs{\states})$ local checks and each local check runs in $O(\abs{\states} \cdot \abs{\act})$ time.
        \item Checking our certificate is in $\logspace(\abs{\states}$).
    \end{enumerate}
\end{restatable}

\begin{remark}
    This is arguably as good as you can be complexity-wise. 
    When checking that the value of every state is correct, you need to touch each state at least once.
    The ranking stuff for lower bounds is necessary, and checking it with one additional operation is about as good as you can get.
\end{remark}

\begin{remark}
    Note that we also claim that the certification should be simple, both in its proof as well as in the process of checking. This is satisfied by our certificates.
\end{remark}


\subsection{Alternative Certificates}
We compare our certificates to alternative certificates in \Cref{app:comparisonAlternativeCerts}.
